Motion Chain of Thought: Disentangling Motion Semantics from Visual Appearance for Robotic Manipulation

World Action Models (WAMs) aim to construct a unified architecture capable of understanding world state evolution and guiding action generation. However, existing visual branches focus on predicting static visual observation, rather than reflecting potential transition information that captures the evolution of world states under motion interactions. This leads to representational entanglement between high-level physical condition evolution and low-level action trajectory generation within the Action Model, creating a structural bottleneck while weakening the predictive capability of world evolution modeling for action generation. We propose PILOT (Physical Inference for Latent Optimized Trajectories), whose core Representational Deduction (RD) bridges this gap by integrating motion chain-of-thought (CoT) guidance as a native model capability. Specifically, RD aims to encourage the action branch to explicitly model potential state transition tokens, which are retained as CoT in the reasoning space to guide fine-grained motion trajectory. Experiments demonstrate that RD not only improves the success rate and generalization ability of WAMs in complex robotic manipulation tasks but also enhances the model's physical interpretability by decoupling high-level motion semantics from low-level trajectory details. Furthermore, the abundant state transition supervision signals introduced by RD effectively alleviate the sparse supervision in action generation, supporting data-efficient real-robot adaptation with reduced demonstration sets.

==> figures/motiv.tex <==
\centering
\centerline{\includegraphics[width=1.0\legacycolumnwidth]{images/motiv.pdf}}
\caption{
Visualization in (a) shows representations of existing WAMs (left) are entangled across actions, and PILOT (right) cleanly clusters by motion semantics. (b) PCA overlay shows PILOT focuses prediction on end-effector-object interaction, while baseline is distracted by background.
}\label{fig:motiv}


==> tables/tab_ablation.tex <==
\begingroup
\setlength{\intextsep}{6pt}
\begin{table}[H]
\input{tables/panel_ablation}
\end{table}
\endgroup

